The New Generation Atlas of Quasar Spectral Energy Distributions from Radio to X-rays

We have produced the next generation of quasar spectral energy distributions (SEDs), essentially updating the work of Elvis et al. (1994) by using high-quality data obtained with several space and ground-based telescopes, including NASA's Great Observatories. We present an atlas of SEDs of 85 optically bright, non-blazar quasars over the electromagnetic spectrum from radio to X-rays. The heterogeneous sample includes 27 radio-quiet and 58 radio-loud quasars. Most objects have quasi-simultaneous ultraviolet-optical spectroscopic data, supplemented with some far-ultraviolet spectra, and more than half also have Spitzer mid-infrared IRS spectra. The X-ray spectral parameters are collected from the literature where available. The radio, far-infrared, and near-infrared photometric data are also obtained from either the literature or new observations. We construct composite spectral energy distributions for radio-loud and radio-quiet objects and compare these to those of Elvis et al., finding that ours have similar overall shapes, but our improved spectral resolution reveals more detailed features, especially in the mid and near-infrared.

==> tab3.online.tex <==
1& MC2 0042+101 &	      74 & 3380 & 390 & VLSS\\
			&&   365 & 540 & 47 & TEXAS\\
			&&  1400 & 218.8 & 7.0 & NVSS\\
			&&  4850 & 83 & 8.1 & GB6\\
2& PG 0052+251 &	    4800 & 0.61 & 0.03 & Leipski.2006\\
			&&  5000 & 0.74 &  & Kellermann.1989\\
			&&  8600 & 0.7 &  & Barvainis.2005\\
3& PKS 0112$-$017 &	      74 & 780 & 120 & VLSS\\
			&&   365 & 974 & 25 & TEXAS\\
			&&   408 & 1110 & 70 & MRC\\
			&&  1400 & 1076.2 & 32.3 & NVSS\\
			&&  4850 & 1437 & 75 & PMN\\
4& 3C 37 &	      74 & 20540 & 2110 & VLSS\\
			&&   178 & 7500 & 938 & 4C\\
			&&   365 & 6936 & 124 & TEXAS\\
			&&   408 & 6070 & 270 & MRC\\
			&&  1400 & 1521.8 & 45.7 & NVSS\\
			&&  4850 & 570 & 50 & GB6\\
5& 3C 47 &	      74 & 67100 & 6760 & VLSS\\
			&&   178 & 26400 & 2110 & 4C\\
			&&   365 & 13016 & 161 & TEXAS\\
			&&  1400 & 3900.7 & 137.4 & NVSS\\
			&&  4850 & 1232 & 110 & GB6\\
			&& 10700 & 600 & 20 & Kellermann.1973\\
			&& 14900 & 360 & 40 & Genzel.1976\\
6& 4C 01.04 &	      74 & 7110 & 740 & VLSS\\
			&&   178 & 3800 & 570 & 4C\\
			&&   365 & 3145 & 70 & TEXAS\\
			&&   408 & 3320 & 150 & MRC\\
			&&  1400 & 1310.5 & 50.3 & NVSS\\
			&&  4850 & 726 & 64 & GB6\\
7& 4C 10.06 &	      74 & 12380 & 1260 & VLSS\\
			&&   178 & 6100 & 763 & 4C\\
			&&   365 & 2205 & 73 & TEXAS\\
			&&   408 & 4060 & 130 & MRC\\
			&&  1400 & 1373.7 & 46.1 & NVSS\\
			&&  4850 & 416 & 37 & GB6\\
8& PKS 0403$-$13 &	      74 & 11190 & 1120 & VLSS\\
			&&   365 & 7621 & 197 & TEXAS\\
			&&   408 & 6700 & 170 & MRC\\
			&&  1400 & 4217.8 & 126.5 & NVSS\\
			&&  4850 & 2738 & 99 & PMN\\
			&& 10700 & 1940 & 70 & Kellermann.1973\\
9& 3C 110 &	      74 & 18230 & 1860 & VLSS\\
			&&   178 & 8000 & 1000 & 4C\\
			&&   365 & 3992 & 93 & TEXAS\\
			&&   408 & 3480 & 160 & MRC\\
			&&  1400 & 765.7 & 26.5 & NVSS\\
			&&  4850 & 342 & 21 & PMN\\
10& 3C 175 &	      74 & 47420 & 4800 & VLSS\\
			&&   178 & 17200 & 1380 & 4C\\
			&&   365 & 10223 & 160 & TEXAS\\
			&&   408 & 8950 & 280 & MRC\\
			&&  1400 & 2643.4 & 87.2 & NVSS\\
			&&  4850 & 678 & 60 & GB6\\
			&& 10700 & 300 & 30 & Kellermann.1973\\
			&& 14900 & 210 & 20 & Genzel.1976\\
11& 3C 186 &	      74 & 32530 & 3250 & VLSS\\
			&&   151 & 15751 & 761 & 7C\\
			&&   178 & 13000 & 1040 & 4C\\
			&&   325 & 7461 & 299 & WENSS\\
			&&   365 & 6582 & 109 & TEXAS\\
			&&  1400 & 1236.4 & 37.1 & NVSS\\
			&&  4850 & 287 & 25 & GB6\\
			&& 10700 & 90 & 15 & Kellermann.1973\\
			&& 14900 & 60 & 10 & Genzel.1976\\
12& B2 0742+31 &	      74 & 14060 & 1430 & VLSS\\
			&&   151 & 5948 & 296 & 7C\\
			&&   178 & 4400 & 770 & 4C\\
			&&   325 & 3458 & 138 & WENSS\\
			&&   365 & 2448 & 64 & TEXAS\\
			&&  1400 & 1357.8 & 41.5 & NVSS\\
			&&  4850 & 958 & 85 & GB6\\
13& IRAS F07546+3928 &	     325 & 155 & 7.8 & WENSS\\
			&&  1400 & 11.56 & 0.58 & FIRST\\
14& 3C 207 &	      74 & 25660 & 2610 & VLSS\\
			&&   178 & 12000 & 960 & 4C\\
			&&   365 & 8922 & 328 & TEXAS\\
			&&   408 & 7030 & 290 & MRC\\
			&&  1400 & 2613.0 & 78.4 & NVSS\\
			&&  4850 & 1166 & 103 & GB6\\
			&& 10700 & 990 & 50 & Kellermann.1973\\
			&& 14900 & 720 & 10 & Genzel.1976\\
15& PG 0844+349 &	    5000 & 0.31 &  & Kellermann.1989\\
16& PKS 0859$-$14 &	      74 & 5070 & 520 & VLSS\\
			&&   365 & 4431 & 93 & TEXAS\\
			&&   408 & 3930 & 180 & MRC\\
			&&  1400 & 2898.1 & 86.9 & NVSS\\
			&&  4850 & 2026 & 99 & PMN\\
			&& 10700 & 1620 & 60 & Kellermann.1973\\
17& 3C 215 &	      74 & 28780 & 2950 & VLSS\\
			&&   178 & 9900 & 1240 & 4C\\
			&&   365 & 5064 & 73 & TEXAS\\
			&&   408 & 6300 & 200 & MRC\\
			&&  1400 & 1586.2 & 51.9 & NVSS\\
			&&  4850 & 459 & 41 & GB6\\
			&& 10700 & 200 & 20 & Kellermann.1973\\
			&& 14900 & 130 & 10 & Genzel.1976\\
18& 4C 39.25 &	      74 & 10920 & 1100 & VLSS\\
			&&   151 & 6685 & 325 & 7C\\
			&&   178 & 5400 & 945 & 4C\\
			&&   325 & 3915 & 157 & WENSS\\
			&&   365 & 3922 & 36 & TEXAS\\
			&&  1400 & 2884.6 & 86.5 & NVSS\\
			&&  4850 & 6614 & 588 & GB6\\
			&&  5000 & 9090 & 100 & Gear.1994\\
			&&  8000 & 11380 & 120 & Gear.1994\\
			&& 14000 & 10150 & 170 & Gear1994\\
19& 4C 40.24 &	      74 & 3210 & 330 & VLSS\\
			&&   151 & 3163 & 162 & 7C\\
			&&   178 & 2500 & 375 & 4C\\
			&&   325 & 2701 & 108 & WENSS\\
			&&   365 & 2940 & 74 & TEXAS\\
			&&  1400 & 1599.5 & 48.0 & NVSS\\
			&&  4850 & 1583 & 141 & GB6\\
20& PG 0947+396 &	    5000 & 0.31 &  & Kellermann.1989\\
21& PG 0953+414 &	    4800 & 0.18 & 0.03 & Leipski.2006\\
			&&  5000 & 1.90 &  & Kellermann.1989\\
22& 4C 55.17 &	      74 & 6470 & 650 & VLSS\\
			&&   151 & 6394 & 323 & 7C\\
			&&   178 & 6400 & 800 & 4C\\
			&&   325 & 4952 & 198 & WENSS\\
			&&   365 & 5255 & 48 & TEXAS\\
			&&  1400 & 3079.2 & 92.4 & NVSS\\
			&&  4850 & 1793 & 159 & GB6\\
			&& 10700 & 1630 & 60 & Kellermann.1973\\
23& 3C 232 &	      74 & 7000 & 740 & VLSS\\
			&&   151 & 5057 & 250 & 7C\\
			&&   178 & 4000 & 1000 & 4C\\
			&&   325 & 3879 & 155 & WENSS\\
			&&   365 & 3625 & 65 & TEXAS\\
			&&  1400 & 1247.1 & 37.4 & NVSS\\
			&&  4850 & 756 & 67 & GB6\\
			&& 10700 & 670 & 30 & Kellermann.1973\\
24& PG 1001+054 &	      74 & 2560 & 280 & VLSS\\
			&&   365 & 739 & 30 & TEXAS\\
			&&  4850 & 58 & 6.6 & GB6\\
			&&  5000 & 0.80 &  & Kellermann.1989\\
25& 4C 22.26 &	      74 & 9860 & 1010 & VLSS\\
			&&   151 & 4630 & 463 & 7C\\
			&&   178 & 3800 & 570 & 4C\\
			&&   365 & 1772 & 54 & TEXAS\\
			&&  1400 & 660.2 & 23.3 & NVSS\\
			&&  4850 & 185 & 16 & GB6\\
26& 4C 41.21 &	      74 & 12130 & 1240 & VLSS\\
			&&   151 & 8710 & 453 & 7C\\
			&&   178 & 6300 & 788 & 4C\\
			&&   325 & 4820 & 193 & WENSS\\
			&&   365 & 4283 & 92 & TEXAS\\
			&&  1400 & 498.1 & 16.9 & NVSS\\
			&&  4850 & 774 & 69 & GB6\\
27& 4C 20.24 &	      74 & 14830 & 1510 & VLSS\\
			&&   151 & 7930 & 793 & 7C\\
			&&   178 & 9500 & 1660 & 4C\\
			&&   365 & 5535 & 132 & TEXAS\\
			&&  1400 & 2493.0 & 87.1 & NVSS\\
			&&  4850 & 1534 & 137 & GB6\\
			&& 10700 & 1080 & 40 & Kellermann.1973\\
28& PG 1100+772 &	      74 & 24150 & 2420 & VLSS\\
			&&   151 & 14853 & 702 & 7C\\
			&&   178 & 10400 & 832 & 4C\\
			&&   325 & 7554 & 302 & WENSS\\
			&&  1400 & 2339.4 & 79.2 & NVSS\\
			&&  5000 & 660 &  & Kellermann.1989\\
29& PG 1103$-$006 &	      74 & 9180 & 960 & VLSS\\
			&&   178 & 4400 & 770 & 4C\\
			&&   365 & 2627 & 63 & TEXAS\\
			&&   408 & 2440 & 70 & MRC\\
			&&  1400 & 1065.6 & 37.1 & NVSS\\
			&&  4850 & 529 & 29 & GB6\\
			&&  5000 & 482 &  & Kellermann.1989\\
30& 3C 254 &	      74 & 51250 & 5210 & VLSS\\
			&&   151 & 28422 & 1459 & 7C\\
			&&   178 & 21700 & 1740 & 4C\\
			&&   325 & 13988 & 560 & WENSS\\
			&&   365 & 12568 & 320 & TEXAS\\
			&&  1400 & 3127.9 & 109.5 & NVSS\\
			&&  4850 & 665 & 59 & GB6\\
			&& 10700 & 320 & 20 & Kellermann.1973\\
			&& 14900 & 200 & 10 & Genzel.1976\\
31& PG 1114+445 &	    5000 & 0.22 &  & Kellermann.1989\\
32& PG 1115+407 &	    1400 & 2.32 & 0.145 & FIRST\\
			&&  5000 & 0.30 &  & Kellermann.1989\\
33& PG 1116+215 &	    1400 & 6.1 & 0.5 & NVSS\\
			&&  1490 & 4.76 & 0.41 & Barvainis.1996\\
			&&  4890 & 2.00 & 0.14 & Barvainis.1996\\
			&&  8480 & 1.23 & 0.09 & Barvainis.1996\\
			&& 14900 & 0.79 & 0.19 & Barvainis.1996\\
34& 4C 12.40 &	      74 & 5980 & 640 & VLSS\\
			&&   178 & 2100 & 525 & 4C\\
			&&   365 & 1376 & 64 & TEXAS\\
			&&   408 & 1170 & 5 & MRC\\
			&&  1400 & 335.8 & 11.7 & NVSS\\
			&&  4850 & 99 & 8.9 & GB6\\
35& PKS 1127$-$14 &	      74 & 3800 & 390 & VLSS\\
			&&   365 & 5379 & 136 & TEXAS\\
			&&   408 & 5070 & 280 & MRC\\
			&&  1400 & 5622.2 & 198.5 & NVSS\\
			&&  4850 & 4316 & 99 & PMN\\
			&& 10700 & 5460 & 180 & Kellermann.1973\\
36& 3C 263 &	      74 & 30140 & 3060 & VLSS\\
			&&   151 & 18054 & 859 & 7C\\
			&&   178 & 13700 & 1100 & 4C\\
			&&   325 & 10759 & 430 & WENSS\\
			&&   365 & 11123 & 262 & TEXAS\\
			&&  1400 & 3290.7 & 108.5 & NVSS\\
			&&  4850 & 1079 & 96 & GB6\\
			&& 10700 & 570 & 20 & Kellermann.1973\\
			&& 14900 & 230 & 20 & Genzel.1976\\
37& MC2 1146+111 &	      74 & 2050 & 230 & VLSS\\
			&&   365 & 567 & 24 & TEXAS\\
			&&  1400 & 172.8 & 6.1 & NVSS\\
			&&  4850 & 56 & 6.3 & GB6\\
38& 4C 49.22 &	      74 & 11090 & 1110 & VLSS\\
			&&   151 & 6907 & 341 & 7C\\
			&&   178 & 5600 & 700 & 4C\\
			&&   325 & 4041 & 162 & WENSS\\
			&&   365 & 3944 & 90 & TEXAS\\
			&&  1400 & 1572.2 & 47.2 & NVSS\\
			&&  4850 & 744 & 66 & GB6\\
39& TEX 1156+213 &	      74 & 2760 & 330 & VLSS\\
			&&   151 & 1280 & 128 & 7C\\
			&&   365 & 328 & 22 & TEXAS\\
			&&  1400 & 270.2 & 9.9 & NVSS\\
			&&  4850 & 102 & 10 & GB6\\
40& PG 1202+281 &	    5000 & 0.83 &  & Kellermann.1989\\
41& 4C 64.15 &	      74 & 4780 & 480 & VLSS\\
			&&   151 & 3143 & 191 & 7C\\
			&&   178 & 2700 & 405 & 4C\\
			&&   325 & 2192 & 88 & WENSS\\
			&&   365 & 2253 & 64 & TEXAS\\
			&&  1400 & 765.1 & 23.0 & NVSS\\
			&&  4850 & 293 & 25 & GB6\\
42& PG 1216+069 &	    1420 & 5.7 & 0.3 & Ulvestad.2005\\
			&&  2270 & 7.1 & 0.4 & Ulvestad.2005\\
			&&  4890 & 9.08 & 0.52 & Barvainis.1996\\
			&&  4990 & 6.4 & 0.3 & Ulvestad.2005\\
			&&  8480 & 12.06 & 0.65 & Barvainis.1996\\
			&& 14900 & 8.36 & 1.2 & Barvainis.1996\\
43& PG 1226+023 &	      74 & 149960 & 15000 & VLSS\\
			&&   178 & 75000 & 6000 & 4C\\
			&&   365 & 66452 & 1908 & TEXAS\\
			&&   408 & 59750 & 1820 & MRC\\
			&&  1400 & 54991.2 & 1900.3 & NVSS\\
			&&  4850 & 44574 & 3972 & GB6\\
			&&  5000 & 38770 & 350 & Gear.1994\\
			&&  8000 & 48140 & 330 & Gear.1994\\
			&& 14000 & 47450 & 510 & Gear1994\\
44& 4C 30.25 &	      74 & 5020 & 510 & VLSS\\
			&&   151 & 2895 & 138 & 7C\\
			&&   178 & 2600 & 390 & 4C\\
			&&   325 & 1903 & 76 & WENSS\\
			&&   365 & 1594 & 70 & TEXAS\\
			&&  1400 & 428.7 & 14.3 & NVSS\\
			&&  4850 & 114 & 11 & GB6\\
45& 3C 277.1 &	      74 & 14720 & 1470 & VLSS\\
			&&   151 & 10701 & 622 & 7C\\
			&&   178 & 8900 & 1110 & 4C\\
			&&   325 & 6792 & 272 & WENSS\\
			&&   365 & 7444 & 172 & TEXAS\\
			&&  1400 & 2288.3 & 68.7 & NVSS\\
			&&  4850 & 776 & 69 & GB6\\
			&& 10700 & 410 & 20 & Kellermann.1973\\
			&& 14900 & 300 & 10 & Genzel.1976\\
46& PG 1259+593 &	    5000 & 0.03 &  & Kellermann.1989\\
47& 3C 281 &	      74 & 12360 & 1270 & VLSS\\
			&&   178 & 5500 & 963 & 4C\\
			&&   365 & 3535 & 80 & TEXAS\\
			&&   408 & 3370 & 160 & MRC\\
			&&  1400 & 1122.0 & 36.1 & NVSS\\
			&&  4850 & 390 & 35 & GB6\\
			&& 10700 & 140 & 16 & Kellermann.1973\\
48& PG 1309+355 &	     151 & 101 & 15.5 & 7C\\
			&&   325 & 102 & 6.2 & WENSS\\
			&&  1400 & 47.2 & 1.5 & NVSS\\
			&&  4850 & 55 & 7.6 & GB6\\
49& PG 1322+659 &	    5000 & 0.20 &  & Kellermann.1989\\
50& 3C 288.1 &	      74 & 15730 & 1570 & VLSS\\
			&&   151 & 11005 & 556 & 7C\\
			&&   178 & 8300 & 1040 & 4C\\
			&&   325 & 5714 & 229 & WENSS\\
			&&   365 & 5069 & 81 & TEXAS\\
			&&  1400 & 1493.3 & 44.8 & NVSS\\
			&&  4850 & 395 & 35 & GB6\\
			&& 10700 & 180 & 30 & Kellermann.1973\\
			&& 14900 & 100 & 10 & Genzel.1976\\
51& PG 1351+640 &	     325 & 45 & 4.7 & WENSS\\
			&&  1400 & 32.7 & 1.1 & NVSS\\
			&&  1420 & 21.3 & 1.1 & Ulvestad.2005\\
			&&  2270 & 14.5 & 0.7 & Ulvestad.2005\\
			&&  4890 & 7.02 & 0.51 & Barvainis.1996\\
			&&  4990 & 6.8 & 0.4 & Ulvestad.2005\\
			&& 14900 & 3.45 & 0.56 & Barvainis.1996\\
52& B2 1351+31 &	      74 & 2040 & 240 & VLSS\\
			&&   151 & 1408 & 112 & 7C\\
			&&   325 & 903 & 36 & WENSS\\
			&&   365 & 1014 & 120 & TEXAS\\
			&&  1400 & 232.1 & 8.2 & NVSS\\
			&&  4850 & 86 & 7.9 & GB6\\
53& PG 1352+183 &	    5000 & 0.25 &  & Kellermann.1989\\
54& 4C 19.44 &	      74 & 15250 & 1560 & VLSS\\
			&&   178 & 7600 & 950 & 4C\\
			&&   365 & 5290 & 81 & TEXAS\\
			&&  1400 & 2585.6 & 88.0 & NVSS\\
			&&  4850 & 2508 & 223 & GB6\\
55& 4C 58.29 &	      74 & 9610 & 980 & VLSS\\
			&&   151 & 4841 & 328 & 7C\\
			&&   178 & 2700 & 405 & 4C\\
			&&   325 & 2335 & 94 & WENSS\\
			&&   365 & 2384 & 62 & TEXAS\\
			&&  1400 & 558.0 & 17.6 & NVSS\\
			&&  4850 & 134 & 12 & GB6\\
56& PG 1402+261 &	    5000 & 0.62 &  & Kellermann.1989\\
57& PG 1411+442 &	    5000 & 0.61 &  & Kellermann.1989\\
58& PG 1415+451 &	    5000 & 0.40 &  & Kellermann.1989\\
59& PG 1425+267 &	      74 & 3310 & 470 & VLSS\\
			&&   151 & 2260 & 226 & 7C\\
			&&   365 & 572 & 64 & TEXAS\\
			&&  1400 & 367.5 & 14.2 & NVSS\\
			&&  4850 & 164 & 15.4 & GB6\\
60& PG 1427+480 &	    5000 & 0.02 &  & Kellermann.1989\\
61& PG 1440+356 &	     151 & 205 & 46.2 & 7C\\
			&&   325 & 81 & 6.5 & WENSS\\
			&&  1400 & 5.2 & 0.4 & NVSS\\
			&&  1490 & 4.46 & 0.10 & Barvainis.1996\\
			&&  4890 & 0.82 & 0.12 & Barvainis.1996\\
			&& 14900 & $<$0.6 &  & Barvainis.1996\\
62& PG 1444+407 &	    5000 & 0.16 &  & Kellermann.1989\\
63& PG 1512+370 &	      74 & 9860 & 1010 & VLSS\\
			&&   151 & 5313 & 281 & 7C\\
			&&   178 & 4800 & 840 & 4C\\
			&&   325 & 3223 & 129 & WENSS\\
			&&   365 & 3003 & 49 & TEXAS\\
			&&  1400 & 988.4 & 31 & NVSS\\
			&&  4850 & 398 & 35 & GB6\\
			&& 10700 & 240 & 20 & Kellermann.1973\\
			&& 15200 & 95 & 10 & Bolton.2004\\
64& PG 1534+580 &	    1400 & 4.8 & 0.4 & NVSS\\
			&&  4800 & 2.21 & 0.05 & Leipski.2006\\
			&&  5000 & 1.92 &  & Kellermann.1989\\
65& PG 1543+489 &	    1400 & 3.6 & 0.5 & NVSS\\
			&&  1490 & 3.20 & 0.57 & Barvainis.1996\\
			&&  4890 & 1.04 & 0.09 & Barvainis.1996\\
			&&  8480 & 0.69 & 0.07 & Barvainis.1996\\
			&& 14900 & $<$0.57 &  & Barvainis.1996\\
66& PG 1545+210 &	      74 & 17750 & 1810 & VLSS\\
			&&   151 & 10440 & 1044 & 7C\\
			&&   178 & 10000 & 1250 & 4C\\
			&&   365 & 5042 & 131 & TEXAS\\
			&&  1400 & 2396.2 & 83.2 & NVSS\\
			&&  4850 & 931 & 82 & GB6\\
			&& 10700 & 400 & 20 & Kellermann.1973\\
67& B2 1555+33 &	      74 & 720 & 100 & VLSS\\
			&&   151 & 533 & 51 & 7C\\
			&&   325 & 339 & 14 & WENSS\\
			&&   365 & 315 & 20 & TEXAS\\
			&&  1400 & 167.2 & 5.7 & NVSS\\
			&&  4850 & 84 & 7.9 & GB6\\
68& B2 1611+34 &	      74 & 1940 & 200 & VLSS\\
			&&   151 & 2709 & 148 & 7C\\
			&&   325 & 2851 & 114 & WENSS\\
			&&   365 & 2928 & 63 & TEXAS\\
			&&  1400 & 4024.1 & 120.7 & NVSS\\
			&&  4850 & 2629 & 234 & GB6\\
			&& 10700 & 2030 & 60 & Kellermann.1973\\
69& 3C 334 &	      74 & 31720 & 3220 & VLSS\\
			&&   178 & 10900 & 872 & 4C\\
			&&   365 & 6708 & 90 & TEXAS\\
			&&   408 & 6800 & 210 & MRC\\
			&&  1400 & 1993.9 & 63.1 & NVSS\\
			&&  4850 & 710 & 63 & GB6\\
			&& 10700 & 330 & 20 & Kellermann.1973\\
			&& 14900 & 310 & 20 & Genzel.1976\\
70& PG 1626+554 &	    5000 & 0.17 &  & Kellermann.1989\\
71& OS 562 &	      74 & 2180 & 270 & VLSS\\
			&&   151 & 1907 & 108 & 7C\\
			&&   325 & 1317 & 53 & WENSS\\
			&&   365 & 1165 & 51 & TEXAS\\
			&&  1400 & 1198.9 & 36.0 & NVSS\\
			&&  4850 & 1607 & 142 & GB6\\
72& PKS 1656+053 &	     365 & 2464 & 69 & TEXAS\\
			&&   408 & 2340 & 110 & MRC\\
			&&  1400 & 1533.8 & 46.0 & NVSS\\
			&&  4850 & 1530 & 136 & GB6\\
73& PG 1704+608 &	      74 & 23580 & 2410 & VLSS\\
			&&   151 & 15330 & 725 & 7C\\
			&&   178 & 13500 & 1080 & 4C\\
			&&   325 & 9540 & 382 & WENSS\\
			&&   365 & 8367 & 284 & TEXAS\\
			&&  1400 & 3259.0 & 124.1 & NVSS\\
			&&  4850 & 1156 & 102 & GB6\\
			&& 10700 & 590 & 30 & Kellermann.1973\\
			&& 14900 & 420 & 20 & Genzel.1976\\
74& MRK 506 &	    1400 & 7.07 & 0.35 & FIRST\\
75& 4C 34.47 &	      74 & 10180 & 1070 & VLSS\\
			&&   151 & 13616 & 772 & 7C\\
			&&   178 & 5000 & 875 & 4C\\
			&&   325 & 4105 & 205 & WENSS\\
			&&   365 & 2467 & 100 & TEXAS\\
			&&  1400 & 1625.6 & 58.9 & NVSS\\
			&&  4850 & 683 & 61 & GB6\\
76& 4C 73.18 &	      74 & 8280 & 860 & VLSS\\
			&&   178 & 3600 & 540 & 4C\\
			&&   325 & 4814 & 193 & WENSS\\
			&&  1400 & 3950.2 & 118.5 & NVSS\\
			&&  4850 & 3688 & 329 & GB6\\
77& MRK 509 &	    1400 & 18.6 & 1.0 & NVSS\\
			&&  1490 & 14.8 & 0.80 & Barvainis.1996\\
			&&  4890 & 5.46 & 0.29 & Barvainis.1996\\
			&& 14900 & 5.14 & 0.38 & Barvainis.1996\\
78& 4C 06.69 &	      74 & 3240 & 330 & VLSS\\
			&&   178 & 3400 & 510 & 4C\\
			&&   365 & 3578 & 48 & TEXAS\\
			&&   408 & 4290 & 190 & MRC\\
			&&  1400 & 2589.1 & 91.4 & NVSS\\
			&&  4850 & 4115 & 366 & GB6\\
			&&  8000 & 7350 & 130 & Gear.1994\\
			&& 14000 & 8450 & 140 & Gear1994\\
79& 4C 31.63 &	      74 & 7100 & 740 & VLSS\\
			&&   178 & 3500 & 525 & 4C\\
			&&   325 & 2837 & 114 & WENSS\\
			&&   365 & 1826 & 73 & TEXAS\\
			&&  1400 & 2933.1 & 100.2 & NVSS\\
			&&  4850 & 2945 & 262 & GB6\\
80& PG 2214+139 &	    5000 & 0.24 &  & Kellermann.1989\\
81& PKS 2216$-$038 &	      74 & 4040 & 420 & VLSS\\
			&&   178 & 2800 & 420 & 4C\\
			&&   365 & 1832 & 73 & TEXAS\\
			&&   408 & 1770 & 50 & MRC\\
			&&  1400 & 2218.2 & 66.5 & NVSS\\
			&&  4850 & 2615 & 99 & PMN\\
82& 3C 446 &	      74 & 25640 & 2570 & VLSS\\
			&&   178 & 17300 & 1380 & 4C\\
			&&   365 & 20231 & 932 & TEXAS\\
			&&   408 & 11890 & 520 & MRC\\
			&&  1400 & 7410.6 & 261.6 & NVSS\\
			&&  4850 & 6485 & 99 & PMN\\
			&& 10700 & 5360 & 150 & Kellermann.1973\\
83& 4C 11.69 &	      74 & 6170 & 620 & VLSS\\
			&&   178 & 5500 & 688 & 4C\\
			&&   365 & 8217 & 88 & TEXAS\\
			&&   408 & 9220 & 200 & MRC\\
			&&  1400 & 7201.5 & 216.0 & NVSS\\
			&&  4850 & 3874 & 345 & GB6\\
			&& 10700 & 2800 & 100 & Kellermann.1973\\
			&& 14900 & 2270 & 20 & Genzel.1976\\
84& PG 2251+113 &	      74 & 11840 & 1240 & VLSS\\
			&&   178 & 6700 & 838 & 4C\\
			&&   365 & 4387 & 89 & TEXAS\\
			&&   408 & 4160 & 110 & MRC\\
			&&  1400 & 1435.8 & 43.1 & NVSS\\
			&&  4850 & 518 & 46 & GB6\\
			&& 10700 & 260 & 30 & Kellermann.1973\\
85& PG 2349$-$014 &	      74 & 15000 & 1530 & VLSS\\
			&&   178 & 6000 & 750 & 4C\\
			&&   365 & 4404 & 108 & TEXAS\\
			&&   408 & 3780 & 120 & MRC\\
			&&  1400 & 1608.4 & 56.2 & NVSS\\
			&&  4850 & 675 & 37 & PMN\\

